Error Analysis and Numerical Algorithm for PDE Approximation with Hidden-Layer Concatenated Physics Informed Neural Networks

We present the hidden-layer concatenated physics informed neural network (HLConcPINN) method, which combines hidden-layer concatenated feed-forward neural networks, a modified block time marching strategy, and a physics informed approach for approximating partial differential equations (PDEs). We analyze the convergence properties and establish the error bounds of this method for two types of PDEs: parabolic (exemplified by the heat and Burgers' equations) and hyperbolic (exemplified by the wave and nonlinear Klein-Gordon equations). We show that its approximation error of the solution can be effectively controlled by the training loss for dynamic simulations with long time horizons. The HLConcPINN method in principle allows an arbitrary number of hidden layers not smaller than two and any of the commonly-used smooth activation functions for the hidden layers beyond the first two, with theoretical guarantees. This generalizes several recent neural-network techniques, which have theoretical guarantees but are confined to two hidden layers in the network architecture and the $\tanh$ activation function. Our theoretical analyses subsequently inform the formulation of appropriate training loss functions for these PDEs, leading to physics informed neural network (PINN) type computational algorithms that differ from the standard PINN formulation. Ample numerical experiments are presented based on the proposed algorithm to validate the effectiveness of this method and confirm aspects of the theoretical analyses.

==> content/auxiliary_proof_wave.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Main Theorems from Section~\ref{Wave}: Wave Equation}\label{Proof}


\noindent\underline{\bf Proof of Theorem \ref{sec5_Theorem1} :}
\begin{proof} Based on Lemma \ref{Ar_7}, there exists a HLConcPINN $u_{\theta_i}$ such that for every $0 \leq m \leq 2$,
	\begin{equation}\label{lem5.1_eq1}
		\|u_{\theta}-u\|_{H^m(\widetilde\Omega_i)}\lesssim {\rm ln}^m(N)N^{-k+m}.
		%\label{lem5.1_eq2}
		%\|v_{\theta}-v\|_{H^s(\widetilde\Omega_i)}\lesssim {\rm ln}^{s}N^{-k+1+s}.
	\end{equation}
	Moreover, by Lemma \ref{Ar_7}, there also exists 
	a HLConcPINN $v_{\theta_i}$ such that for every $0 \leq s \leq 2$,
	\begin{align}
		\label{lem5.1_eq2}
		\|v_{\theta}-v\|_{L^2(\widetilde\Omega_i)}\lesssim {\rm ln}^{s}N^{-k+1}\qquad
		\|v_{\theta}-v\|_{H^1(\widetilde\Omega_i)}\lesssim {\rm ln}^{s}N^{-k+2}.
	\end{align}
	According to Lemma \ref{Ar_2}, we can bound the HLConcPINN residual terms,
	\begin{align*}
		&\|\frac{\partial \hat{u}_i}{\partial t}\|_{L^2(\widetilde\Omega_i)}\leq\|\hat{u}_i\|_{H^1(\widetilde\Omega_i)},\qquad
		\|\frac{\partial \hat{v}_i}{\partial t}\|_{L^2(\widetilde\Omega_i)}\leq\|\hat{v}_i\|_{H^1(\widetilde\Omega_i)},\\
		&\|\Delta\hat{u}_i\|_{L^2(\widetilde\Omega_i)}\leq\|\hat{u}_i\|_{H^2(\widetilde\Omega_i)},\qquad
		\|\nabla\frac{\partial \hat{u}_i}{\partial t}\|_{L^2(\widetilde\Omega_i)}\leq\|\hat{u}_i\|_{H^2(\widetilde\Omega_i)},\qquad
		\|\nabla\hat{v}_i\|_{L^2(\widetilde\Omega_i)}\leq\|\hat{v}_i\|_{H^1(\widetilde\Omega_i)},\\
		&\|\hat{u}_i\|_{L^2(D)}\leq \|\hat{u}_i\|_{L^2(\partial\widetilde\Omega_i)}\leq C_{h_{\widetilde\Omega_i},d+1,\rho_{\widetilde\Omega_i}}\|\hat{u}_i\|_{H^1(\widetilde\Omega_i)},\\
		&\|\hat{v}_i\|_{L^2(D)}\leq \|\hat{v}_i\|_{L^2(\partial\widetilde\Omega_i)}\leq C_{h_{\widetilde\Omega_i},d+1,\rho_{\widetilde\Omega_i}}\|\hat{v}_i\|_{H^1(\widetilde\Omega_i)},\\
		&\|\nabla\hat{u}_i\|_{L^2(D)}\leq \|\nabla\hat{u}_i\|_{L^2(\partial\widetilde\Omega_i)}\leq C_{h_{\widetilde\Omega_i},d+1,\rho_{\widetilde\Omega_i}}\|\hat{u}_i\|_{H^2(\widetilde\Omega_i)},\\
		&\|\hat{v}_i\|_{L^2(\widetilde\Omega_{*i})}\leq \|\hat{v}_i\|_{L^2(\partial\widetilde\Omega_i)}\leq C_{h_{\widetilde\Omega_i},d+1,\rho_{\widetilde\Omega_i}}\|\hat{v}_i\|_{H^1(\widetilde\Omega_i)},\\
		&\|\nabla\hat{u}_i\|_{L^2(\widetilde\Omega_{*i})}\leq \|\nabla\hat{u}_i\|_{L^2(\partial\widetilde\Omega_i)}\leq C_{h_{\widetilde\Omega_i},d+1,\rho_{\widetilde\Omega_i}}\|\hat{u}_i\|_{H^2(\widetilde\Omega_i)}.
	\end{align*}
	For $j=1$, $R_{tb1_{i}}|_{t=t_{0}}=\hat{u}_{i}|_{t=t_{0}}$ and $R_{tb2_{i}}|_{t=t_{0}}=\hat{v}_{i}|_{t=t_{0}}$, we obtain
	\begin{align*}
		&\|R_{tb1_{i}}(\bm{x},0)\|_{L^2(D)}\leq\|\hat{u}_i\|_{L^2(\partial\widetilde\Omega_{i})}\leq C_{h_{\widetilde\Omega_{i}},d+1,\rho_{\widetilde\Omega_{i}}}\|\hat{u}_i\|_{H^1(\widetilde\Omega_{i})},\\
		&\|R_{tb2_{i}}(\bm{x},0)\|_{L^2(D)}\leq\|\hat{v}_i\|_{L^2(\partial\widetilde\Omega_{i})}\leq C_{h_{\widetilde\Omega_{i}},d+1,\rho_{\widetilde\Omega_{i}}}\|\hat{v}_i\|_{H^1(\widetilde\Omega_{i})}.
	\end{align*}
	For $j>1$, it holds 
	\begin{align*}
		&\|R_{tb1_{i}}(\bm{x},t_{j-1})\|_{L^2(D)}%=\|\hat{u}_{i}|_{t=t_{j-1}}-\hat{u}_{j-1}|_{t=t_{j-1}}\|_{L^2(D)}
		\leq \|\hat{u}_{i}|_{t=t_{j-1}}\|_{L^2(D)}+\|\hat{u}_{j-1}|_{t=t_{j-1}}\|_{L^2(D)}
		\leq\|\hat{u}_i\|_{L^2(\partial\widetilde\Omega_{j-1})}+\|\hat{u}_{j-1}\|_{L^2(\partial\widetilde\Omega_{j-1})}\\
		&\quad\leq C_{h_{\widetilde\Omega_{j-1}},d+1,\rho_{\widetilde\Omega_{j-1}}}(\|\hat{u}_i\|_{H^1(\widetilde\Omega_{j-1})}+\|\hat{u}_{j-1}\|_{H^1(\widetilde\Omega_{j-1})})\leq  C_{h_{\widetilde\Omega_{j-1}},d+1,\rho_{\widetilde\Omega_{j-1}}}(\|\hat{u}_i\|_{H^1(\widetilde\Omega_{i})}+\|\hat{u}_{j-1}\|_{H^1(\widetilde\Omega_{j-1})}).
	\end{align*} 
	Similarly, 
	\[
	\|R_{tb2_{i}}(\bm{x},t_{j-1})\|_{L^2(D)}\leq  C_{h_{\widetilde\Omega_{j-1}},d+1,\rho_{\widetilde\Omega_{j-1}}}(\|\hat{v}_i\|_{H^1(\widetilde\Omega_{i})}+\|\hat{v}_{j-1}\|_{H^1(\widetilde\Omega_{j-1})}).
	\]
	By combining these relations with \eqref{lem5.1_eq1} and \eqref{lem5.1_eq2},
	we can obtain
	% Based on the definition of $\beta$, it should be >1.
	\begin{align*}
		&\|R_{int1_{i}}\|_{L^2(\widetilde\Omega_i)}=\|\frac{\partial \hat{u}_i}{\partial t}-\hat{v}_i\|_{L^2(\widetilde\Omega_i)}\leq
		\|\hat{u}_i\|_{H^1(\widetilde\Omega_i)}+\|\hat{v}_i\|_{L^2(\widetilde\Omega_i)}%\\
		%&\quad\leq C_{1,k,d+1,u}\lambda_{1,u}(N)N^{-k+1} + C_{0,k-1,d+1,v}\lambda_{0,v}(N)N^{-k+1}
		\lesssim {\rm ln}NN^{-k+1},\\
		&\|R_{int2_{i}}\|_{L^2(\widetilde\Omega_i)}=\|\frac{\partial \hat{v}_i}{\partial t}-\Delta\hat{u}_i\|_{L^2(\widetilde\Omega_i)}\leq
		\|\hat{v}_i\|_{H^1(\widetilde\Omega_i)}+\|\hat{u}_i\|_{H^2(\widetilde\Omega_i)}%\\
		%&\quad\leq C_{2,k,d+1,u}\lambda_{2,u}(N)N^{-k+2} + C_{1,k-1,d+1,v}\lambda_{1,v}(N)N^{-k+2}
		\lesssim {\rm ln}^2NN^{-k+2},\\		
		&\|\nabla R_{int1_{i}}\|_{L^2(\widetilde\Omega_i)}=\|\nabla(\frac{\partial \hat{u}_i}{\partial t}-\hat{v}_i)\|_{L^2(\widetilde\Omega_i)}\leq
		\|\hat{u}_i\|_{H^2(\widetilde\Omega_i)}+\|\hat{v}_i\|_{H^1(\widetilde\Omega_i)}%\\
		%&\quad\leq C_{2,k,d+1,u}\lambda_{2,u}(N)N^{-k+2} + C_{1,k-1,d+1,v}\lambda_{1,v}(N)N^{-k+2}
		\lesssim {\rm ln}^2NN^{-k+2},\\
		&\|R_{tb1_{i}}\|_{L^2(D)}\leq C_{h_{\widetilde\Omega_i},d+1,\rho_{\widetilde\Omega_i}}\|\hat{u}_i\|_{H^1(\widetilde\Omega_i)}\lesssim {\rm ln}NN^{-k+1},\\	
		&\|R_{tb2_{i}}\|_{L^2(D)}, \|R_{sb1_{i}}\|_{L^2(\widetilde\Omega_{*i})}\leq C_{h_{\widetilde\Omega_i},d+1,\rho_{\widetilde\Omega_i}}\|\hat{v}_i\|_{H^1(\widetilde\Omega_i)}\lesssim {\rm ln}NN^{-k+2},\\	
		&\|\nabla R_{tb1_{i}}\|_{L^2(D)}, \|R_{sb2_{i}}\|_{L^2(\widetilde\Omega_{*i})}\leq C_{h_{\widetilde\Omega_i},d+1,\rho_{\widetilde\Omega_i}}\|\hat{u}_i\|_{H^2(\widetilde\Omega_i)}\lesssim {\rm ln}^2NN^{-k+2}.
	\end{align*}
	Then, we finish our proof.
\end{proof}

\vspace{0.1in}
\noindent\underline{\bf Proof of Theorem \ref{sec5_Theorem2} :}
\begin{proof} Taking the $L^2$ inner product of \eqref{wave_error_eq1} and \eqref{wave_error_eq2} with $\hat{u}_i$ and $\hat{v}_i$ over $D$, respectively, we have
	\begin{align}
		\label{sec5_eq0}
		&\frac{d}{2dt}\int_{D} |\hat{u}_i|^2\dx = \int_{D}\hat{u}_i\hat{v}_i\dx+\int_{D} R_{int1_{i}}\hat{u}_i\dx\leq \int_{D} |\hat{u}_i|^2\dx+\frac{1}{2}\int_{D} |R_{int1_{i}}|^2\dx+\frac{1}{2}\int_{D} |\hat{v}_i|^2\dx,\\
		\label{sec5_eq1}
		&\frac{d}{2dt}\int_{D} |\hat{v}_i|^2\dx =- \int_{D}\nabla\hat{u}_i\cdot\nabla\hat{v}_i\dx+\int_{\partial D} \hat{v}_i\nabla\hat{u}_i\cdot\bm{n}\ds+\int_{D} R_{int2_{i}}\hat{v}_i\dx
		\nonumber\\
		%&=- \int_{D}\nabla\hat{u}_i\cdot\nabla\frac{\partial \hat{u}_i}{\partial t}\dx+\int_{D}\nabla\hat{u}_i\cdot\nabla R_{int1_{i}}\dx+\int_{\partial D} \hat{v}_i\nabla\hat{u}_i\cdot\bm{n}\ds+\int_{D} R_{int2_{i}}\hat{v}_i\dx\nonumber\\
		&\quad=-\frac{d}{2dt}\int_{D} |\nabla\hat{u}_i|^2\dx 
		+\int_{D}\nabla\hat{u}_i\cdot\nabla R_{int1_{i}}\dx
		+\int_{\partial D} \hat{v}_i\nabla\hat{u}_i\cdot\bm{n}\ds
		+\int_{D} R_{int2_{i}}\hat{v}_i\dx
		\nonumber\\
		&\quad\leq-\frac{d}{2dt}\int_{D} |\nabla\hat{u}_i|^2\dx +\frac{1}{2}\int_{D} |\nabla\hat{u}_i|^2\dx+\frac{1}{2}\int_{D} |\nabla R_{int1_{i}}|^2\dx+C_{\partial D_{1i}}(\int_{\partial D}|R_{sb1_{i}}|^2\ds)^{1/2}
		\nonumber\\
		&\qquad+C_{\partial D_{2i}}(\int_{\partial D}|R_{sb2_{i}}|^2\ds)^{1/2}+\frac{1}{2}\int_{D} |\hat{v}_i|^2\dx+\frac{1}{2}\int_{D} |R_{int2_{i}}|^2\dx.
	\end{align}
	Here, we have used $\hat{v}_i=\frac{\partial \hat{u}_i}{\partial t}-R_{int1_{i}}$, $C_{\partial D_{1i}}=|\partial D|^{\frac{1}{2}}(\|u\|_{C^1(\partial D\times[0,t_i])}+\|u_{\theta_i}\|_{C^1(\partial D\times[0,t_i])})$ and
 $C_{\partial D_{2i}}=|\partial D|^{\frac{1}{2}}(\|v\|_{C(\partial D\times [0,t_i])}+\|v_{\theta_i}\|_{C(\partial D\times [0,t_i])})$. By adding \eqref{sec5_eq0} to \eqref{sec5_eq1}, we have
	\begin{align}\label{sec5_eq2}
		&\frac{d}{2dt}\int_{D} |\hat{u}_i|^2\dx+\frac{d}{2dt}\int_{D} |\nabla\hat{u}_i|^2\dx +\frac{d}{2dt}\int_{D} |\hat{v}_i|^2\dx
		\nonumber\\
		&\qquad \leq \int_{D} |\hat{u}_i|^2\dx+\frac{1}{2}\int_{D} |\nabla\hat{u}_i|^2\dx+\int_{D} |\hat{v}_i|^2\dx+\frac{1}{2}\int_{D} |R_{int1_{i}}|^2\dx+\frac{1}{2}\int_{D} |R_{int2_{i}}|^2\dx
		\nonumber\\
		&\qquad+\frac{1}{2}\int_{D} |\nabla R_{int1_{i}}|^2\dx+C_{\partial D_{1i}}(\int_{\partial D}|R_{sb1_{i}}|^2\ds)^{1/2}+C_{\partial D_{2i}}(\int_{\partial D}|R_{sb2_{i}}|^2\ds)^{1/2}.
	\end{align}
	Integrating \eqref{sec5_eq2} over $[t_{i-1},\tau]$ for any $t_{i-1}<\tau \leq t_i$, using the initial conditions \eqref{wave_error_eq3} and \eqref{wave_error_eq4}, and applying the Cauchy–Schwarz inequality, we obtain
    \begin{align*}
		&\int_{D} |\hat{u}_i(\bm{x},\tau)|^2\dx 
		+\int_{D} |\nabla\hat{u}_i(\bm{x},\tau)|^2\dx
		+\int_{D} |\hat{v}_i(\bm{x},\tau)|^2\dx
		\nonumber\\
		&\quad\leq\int_{D}(|\hat{u}_i(\bm{x},t_{i-1})|^2+|\hat{v}_i(\bm{x},t_{i-1})|^2+|\nabla\hat{u}_i(\bm{x},t_{i-1})|^2)\dx
		+2\int_{\Omega_i}\left(|\hat{u}_i|^2+ |\nabla\hat{u}_i|^2+ |\hat{v}_i|^2 \right)\dx\dt
		\nonumber\\
		&\qquad+ \int_{\Omega_i}\left(|R_{int1_{i}}|^2+|R_{int2_{i}}|^2+|\nabla R_{int1_{i}}|^2\right)\dx\dt+2C_{\partial D_{1i}}|\Delta t|^{1/2}(\int_{\Omega_{*i}}|R_{sb1_{i}}|^2\ds\dt)^{1/2}\nonumber\\
		&\qquad+2C_{\partial D_{2i}}|\Delta t|^{1/2}(\int_{\Omega_{*i}}|R_{sb2_{i}}|^2\ds\dt)^{1/2}
		\nonumber\\
		&\quad\leq\int_{D}(|\hat{u}_i(\bm{x},t_{i-1})|^2+|\hat{v}_i(\bm{x},t_{i-1})|^2+|\nabla\hat{u}_i(\bm{x},t_{i-1})|^2)\dx
		+2\int_{\Omega_i} \left(|\hat{u}_i|^2+ |\nabla\hat{u}_i|^2+ |\hat{v}_i|^2 \right)\dx\dt
		\nonumber\\
		&\qquad+ \int_{\Omega_i}\left(|R_{int1_{i}}|^2+|R_{int2_{i}}|^2+|\nabla R_{int1_{i}}|^2\right)\dx\dt+2C_{\partial D_{1i}}|\Delta t|^{1/2}(\int_{\Omega_{*i}}|R_{sb1_{i}}|^2\ds\dt)^{1/2}
        \nonumber\\
		&\qquad+2C_{\partial D_{2i}}|\Delta t|^{1/2}(\int_{\Omega_{*i}}|R_{sb2_{i}}|^2\ds\dt)^{1/2}
		+\sum_{j=1}^{i-1}\int_{D}(|R_{tb1_{i}}(\bm{x},t_{j-1})|^2+|R_{tb2_{i}}(\bm{x},t_{j-1})|^2)\dx
        \nonumber\\
		&\qquad
		+\sum_{j=1}^{i-1}\int_{D}|\nabla R_{tb1_{i}}(\bm{x},t_{j-1})|^2\dx
		\nonumber\\
		&\quad\leq 2\int_{D}(|\hat{u}_{i-1}(\bm{x},t_{i-1})|^2+|\hat{v}_{i-1}(\bm{x},t_{i-1})|^2+|\nabla\hat{u}_{i-1}(\bm{x},t_{i-1})|^2)\dx+2\int_{\Omega_i}\left(|\hat{u}_i|^2+ |\nabla\hat{u}_i|^2+ |\hat{v}_i|^2 \right)\dx\dt
		\nonumber\\
		&\qquad+ \int_{\Omega_i}\left(|R_{int1_{i}}|^2+|R_{int2_{i}}|^2+|\nabla R_{int1_{i}}|^2\right)\dx\dt+2C_{\partial D_{1i}}|\Delta t|^{1/2}(\int_{\Omega_{*i}}|R_{sb1_{i}}|^2\ds\dt)^{1/2}
        \nonumber\\
		&\qquad+2C_{\partial D_{2i}}|\Delta t|^{1/2}(\int_{\Omega_{*i}}|R_{sb2_{i}}|^2\ds\dt)^{1/2}
		+2\sum_{j=1}^{i}\int_{D}(|R_{tb1_{i}}(\bm{x},t_{j-1})|^2+|R_{tb2_{i}}(\bm{x},t_{j-1})|^2)\dx
        \nonumber\\
		&\qquad
		+2\sum_{j=1}^{i}\int_{D}|\nabla R_{tb1_{i}}(\bm{x},t_{j-1})|^2\dx.
	\end{align*}
	Then, applying the integral form of the Gr${\rm\ddot{o}}$nwall inequality to the above inequality, it holds
	\begin{align}\label{sec5_eq3}
        &\int_{D} \left(|\hat{u}_i(\bm{x},\tau)|^2+|\nabla\hat{u}_i(\bm{x},\tau)|^2+|\hat{v}_i(\bm{x},\tau)|^2\right)\dx
        \nonumber\\
       &\quad\leq2\int_{D}(|\hat{u}_{i-1}(\bm{x},t_{i-1})|^2+|\hat{v}_{i-1}(\bm{x},t_{i-1})|^2+|\nabla\hat{u}_{i-1}(\bm{x},t_{i-1})|^2)\dx\exp(2\Delta t)
       \nonumber\\
	   &\qquad +\int_{\Omega_i}(|R_{int1_{i}}|^2+|R_{int2_{i}}|^2+|\nabla R_{int1_{i}}|^2)\dx\dt\exp(2\Delta t)%+\int_{\Omega_{*i}}(|R_{sb1_{i}}|^2+|R_{sb2_{i}}|^2)\ds\dt\exp(2\Delta t)
       \nonumber\\
       &\qquad +2|\Delta t|^{1/2}\big(C_{\partial D_{1i}}(\int_{\Omega_{*i}}|R_{sb1_{i}}|^2\ds\dt)^{1/2}+C_{\partial D_{2i}}(\int_{\Omega_{*i}}|R_{sb2_{i}}|^2\ds\dt)^{1/2}\big)\exp(2\Delta t)
       \nonumber\\
	   &\qquad +2\sum_{j=1}^i\int_{D}(|R_{tb1_{i}}(\bm{x},t_{j-1})|^2+|R_{tb2_{i}}(\bm{x},t_{j-1})|^2+|\nabla R_{tb1_{i}}(\bm{x},t_{j-1})|^2)\dx\exp(2\Delta t).
	\end{align}
 
	For $i=1$, it is easily to get the result \eqref{lem5.4}. And then, we can obtain \eqref{lem5.5} by integrating the above inequality over $[t_{0},t_{1}]$.
	
	Next, we assume that Theorem \ref{sec5_Theorem2} holds for all $\tau \in [t_{i-1},
	t_i]$ and $2\leq i\leq l-1$, i.e.,
	\begin{align*}
		&\int_{D}(|\hat{u}_i(\bm{x},\tau)|^2+|\nabla\hat{u}_i(\bm{x},\tau)|^2+|\hat{v}_i(\bm{x},\tau)|^2)\dx\leq C_{G_{i}}\exp(2\Delta t),\\
		&\int_{t_{i-1}}^{t_{i}}\int_{D}(|\hat{u}_i(\bm{x},t)|^2+|\nabla\hat{u}_i(\bm{x},t)|^2+|\hat{v}_i(\bm{x},t)|^2)\dx\dt\leq C_{G_{i}}\Delta t\exp(2\Delta t). 
	\end{align*}
	
	Last, we need to prove that Theorem \ref{sec5_Theorem2}  is true at $i=l$. Combining the above inequalities and \eqref{sec5_eq3} for $i=l$, we have
	\begin{align*}
		&\int_{D} \left(|\hat{u}_l(\bm{x},\tau)|^2+|\nabla\hat{u}_l(\bm{x},\tau)|^2+|\hat{v}_l(\bm{x},\tau)|^2\right)\dx\nonumber\\
		&\quad\leq2\int_{D}(|\hat{u}_{l-1}(\bm{x},t_{l-1})|^2+|\hat{v}_{l-1}(\bm{x},t_{l-1})|^2+|\nabla\hat{u}_{l-1}(\bm{x},t_{l-1})|^2)\dx\exp(2\Delta t)\nonumber\\
		&\qquad +\int_{\Omega_l}(|R_{int1_{l}}|^2+|R_{int2_{l}}|^2+|\nabla R_{int1_{l}}|^2)\dx\dt\exp(2\Delta t)
        \nonumber\\
   	  &\qquad +2|\Delta t|^{1/2}\big(C_{\partial D_{1l}}(\int_{\Omega_{*l}}|R_{sb1_{l}}|^2\ds\dt)^{1/2}+C_{\partial D_{2l}}(\int_{\Omega_{*l}}|R_{sb2_{l}}|^2\ds\dt)^{1/2}\big)\exp(2\Delta t)
        \nonumber\\
		&\qquad +2\sum_{j=1}^l\int_{D}(|R_{tb1_{l}}(\bm{x},t_{j-1})|^2+|R_{tb2_{l}}(\bm{x},t_{j-1})|^2+|\nabla R_{tb1_{l}}(\bm{x},t_{j-1})|^2)\dx\exp(2\Delta t)\nonumber\\
		&\quad\leq 2C_{G_{l-1}}\exp(2\Delta t)+\widetilde{C}_{G_{l}}\exp(2\Delta t)=C_{G_{l}}\exp(2\Delta t),\nonumber\\
		&\int_{t_{l-1}}^{t_l}\int_{D} \left(|\hat{u}_l(\bm{x},t)|^2+|\nabla\hat{u}_l(\bm{x},t)|^2+|\hat{v}_l(\bm{x},t)|^2\right)\dx\dt\leq C_{G_{l}}\Delta t\exp(2\Delta t).
	\end{align*}
	By using the mathematical induction and deduction methods, we finish the proof.
\end{proof} 

\vspace{0.1in}
\noindent\underline{\bf Proof of Theorem \ref{sec5_Theorem3} :}
\begin{proof} By the quadrature error formula \eqref{int1}, we have
	\begin{align*}
		&\int_{D}|R_{tb1_{i}}|^2\dx=\int_{D}|R_{tb1_{i}}|^2\dx-\mathcal{Q}_{M_{tb_{i}}}^{D}(R_{tb1_{i}}^2)+\mathcal{Q}_{M_{tb_{i}}}^{D}(R_{tb1_{i}}^2)
		\leq C_{({R_{tb1_{i}}^2})}M_{tb_{i}}^{-\frac{2}{d}}+\mathcal{Q}_{M_{tb_{i}}}^{D}(R_{tb1_{i}}^2),\\
		&\int_{D}|R_{tb2_{i}}|^2\dx=\int_{D}|R_{tb2_{i}}|^2\dx-\mathcal{Q}_{M_{tb_{i}}}^{D}(R_{tb2_{i}}^2)+\mathcal{Q}_{M_{tb_{i}}}^{D}(R_{tb2_{i}}^2)
		\leq C_{({R_{tb2_{i}}^2})}M_{tb_{i}}^{-\frac{2}{d}}+\mathcal{Q}_{M_{tb_{i}}}^{D}(R_{tb2_{i}}^2),\\
		&\int_{D}|\nabla R_{tb1_{i}}|^2\dx=\int_{D}|\nabla R_{tb1_{i}}|^2\dx-\mathcal{Q}_{M_{tb_{i}}}^{D}(|\nabla R_{tb1_{i}}|^2)+\mathcal{Q}_{M_{tb_{i}}}^{D}(|\nabla R_{tb1_{i}}|^2)
		\leq C_{(|\nabla R_{tb1_{i}}|^2)}M_{tb_{i}}^{-\frac{2}{d}}+\mathcal{Q}_{M_{tb_{i}}}^{D}(|\nabla R_{tb1_{i}}|^2),\\
		&\int_{\Omega_{i}}|R_{int1_{i}}|^2\dx\dt=\int_{\Omega_{i}}|R_{int1_{i}}|^2\dx\dt-\mathcal{Q}_{M_{int_{i}}}^{\Omega_i}(R_{int1_{i}}^2)+\mathcal{Q}_{M_{int_{i}}}^{\Omega_i}(R_{int1_{i}}^2)
		\leq C_{({R_{int1_{i}}^2})}M_{int_{i}}^{-\frac{2}{d+1}}+\mathcal{Q}_{M_{int_{i}}}^{\Omega_i}(R_{int1_{i}}^2),\\
		&\int_{\Omega_{i}}|R_{int2_{i}}|^2\dx\dt=\int_{\Omega_{i}}|R_{int2_{i}}|^2\dx\dt-\mathcal{Q}_{M_{int_{i}}}^{\Omega_i}(R_{int2_{i}}^2)+\mathcal{Q}_{M_{int_{i}}}^{\Omega_i}(R_{int2_{i}}^2)
		\leq C_{(R_{int2_{i}}^2)}M_{int_{i}}^{-\frac{2}{d+1}}+\mathcal{Q}_{M_{int_{i}}}^{\Omega_i}(R_{int2_{i}}^2),\\
		&\int_{\Omega_{i}}|\nabla R_{int1_{i}}|^2\dx\dt=\int_{\Omega_{i}}|\nabla R_{int1_{i}}|^2\dx\dt-\mathcal{Q}_{M_{int_{i}}}^{\Omega_i}(|\nabla R_{int1_{i}}|^2)+\mathcal{Q}_{M_{int_{i}}}^{\Omega_i}(|\nabla R_{int1_{i}}|^2)\\
		&\qquad\qquad
		\leq C_{(|\nabla R_{int1_{i}}|^2)}M_{int_{i}}^{-\frac{2}{d+1}}+\mathcal{Q}_{M_{int_{i}}}^{\Omega_i}(|\nabla R_{int1_{i}}|^2),\\
		&\int_{\Omega_{*i}}|R_{sb1_{i}}|^2\ds\dt=\int_{\Omega_{*i}}|R_{sb1_{i}}|^2\ds\dt-\mathcal{Q}_{M_{sb_{i}}}^{\Omega_{*i}}(R_{sb1_{i}}^2)+\mathcal{Q}_{M_{sb_{i}}}^{\Omega_{*i}}(R_{sb1_{i}}^2)
		\leq C_{({R_{sb1_{i}}^2})}M_{sb_{i}}^{-\frac{2}{d}}+\mathcal{Q}_{M_{sb_{i}}}^{\Omega_{*i}}(R_{sb1_{i}}^2),\\
		&\int_{\Omega_{*i}}|R_{sb2_{i}}|^2\ds\dt=\int_{\Omega_{*i}}|R_{sb2_{i}}|^2\ds\dt-\mathcal{Q}_{M_{sb_{i}}}^{\Omega_{*i}}(R_{sb2_{i}}^2)+\mathcal{Q}_{M_{sb_{i}}}^{\Omega_{*i}}(R_{sb2_{i}}^2)
		\leq C_{({R_{sb2_{i}}^2})}M_{sb_{i}}^{-\frac{2}{d}}+\mathcal{Q}_{M_{sb_{i}}}^{\Omega_{*i}}(R_{sb2_{i}}^2).
	\end{align*}
	Combining the fact that $C_{(R_{tb1_{i}}^2)}\lesssim\|R_{tb1_{i}}^2\|_{C^2}$ and $\|R_{tb1_{i}}^2\|_{C^n}\leq 2^n\|R_{tb1_{i}}\|_{C^n}^2$ with Lemma \ref{Ar_3}, it holds
	\begin{align}\label{sec5_eq4}
		&C_{(R_{tb1_{i}}^2(\bm{x},t_{j-1}))}\lesssim\|R_{tb1_{i}}(\bm{x},t_{j-1})\|_{C^2}^2\leq 2(\|\hat{u}_{i}|_{t=t_{j-1}} \|_{C^2}^2+\|\hat{u}_{j-1}|_{t=t_{j-1}} \|_{C^2}^2)
		\nonumber\\
		&\qquad\lesssim \|u\|_{C^2}^2+(e^2n^4W^3R^n\|\sigma\|_{C^2(\Omega)})^{4L}.
	\end{align}
	
	In a similar way, we can estimate the terms $\int_{D}|R_{tb2_{i}}|^2\dx$, $\int_{D}|\nabla R_{tb1_{i}}|^2\dx$, 
	$\int_{\Omega_{i}}|R_{int1_{i}}|^2\dx\dt$, $\int_{\Omega_{i}}|R_{int2_{i}}|^2\dx\dt$,  $\int_{\Omega_{i}}|\nabla R_{int1_{i}}|^2\dx\dt$, $\int_{\Omega_{*i}}|R_{sb1_{i}}|^2\ds\dt$ and $\int_{\Omega_{*i}}|R_{sb2_{i}}|^2\ds\dt$. 
	
	Combining the above inequalities with Theorem \ref{sec5_Theorem2}, it holds that
	\begin{equation*}
		\int_{t_{i-1}}^{t_{i}}\int_{D}(|\hat{u}_i(\bm{x},t)|^2+|\nabla \hat{u}_i(\bm{x},t)|^2+|\hat{v}_i(\bm{x},t)|^2)\dx\dt\leq  C_{T_i}\Delta t\exp(2\Delta t),
	\end{equation*}
	where the constant $C_{T_i}$ is defined in \eqref{sec5_eq5}. Here, $C_{R_q^2}$ can be estimated using a method similar to \eqref{sec5_eq4} with $R_q$ taking $R_{tb1_{i}}$, $R_{tb2_{i}}$, $\nabla R_{tb1_{i}}$, $R_{int1_{i}}$, $R_{int2_{i}}$, $\nabla R_{int1_{i}}$, $R_{sb1_{i}}$ and $R_{sb2_{i}}$.
\end{proof} 


